Particle acceleration in explosive relativistic reconnection events and Crab Nebula gamma-ray flares

We develop a model of gamma-ray flares of the Crab Nebula resulting from the magnetic reconnection events in highly-magnetized relativistic plasma. We first discuss physical parameters of the Crab nebula and review the theory of pulsar winds and termination shocks. We also review the principle points of particle acceleration in explosive reconnection events (Lyutikov et al. 2017a,b). It is required that particles producing flares are accelerated in highly magnetized regions of the nebula. Flares originate from the poleward regions at the base of Crab's polar outflow, where both the magnetization and the magnetic field strength are sufficiently high. The post-termination shock flow develops macroscopic (not related to the plasma properties on the skin-depth scale) kink-type instabilities. The resulting large-scales magnetic stresses drive explosive reconnection events on the light-crossing time of the reconnection region. Flares are produced at the initial stage of the current sheet development, during the X-point collapse. The model has all the ingredients needed for Crab flares: natural formation of highly magnetized regions, explosive dynamics on light travel time, development of high electric fields on macroscopic scales and acceleration of particles to energies well exceeding the average magnetic energy per particle.

==> AlfvenCurrent_.tex <==

%sssssssssss
\subsection{Potential-Luminosity relationship and the \Alfven current}

There is Êan important, yet somewhat subtle,  relationship between the parameters of the flares that serve as a confirmation of the basic principles of our approach, as we discuss next.  In addition to particle acceleration the reconnecting \Ef\ 
 also drives (a charge-separated) current.  That induced current creates its own \Bf; particle gyration in the induced \Bf\ can inhibit the beam propagation. 
 These considerarations place an upper limit on the total charger-separated current, known as the \Alfven current.
 The relativistic  \Alfven current \citep{1939PhRv...55..425A,1973PhFl...16.1298L} is
\be
I_A = \gamma {m_e c^3 \over e}.
\label{IA}
\ee

In the present model of Crab flares, the reconnection events result in a population of $\gamma$-ray emitting particles

Now, using the total flare luminosity and the estimates of the energy of emitting particles we can verify that the current carried by the flare-emitting particles does violate the \Alfven limit.


 Qualitatively,  the \EM\ power of relativistic outflows can be estimated as  \citep{BlandfordZnajek,2002luml.conf..381B} 
\be 
L_{EM} \approx V^2 /{\cal{R}}
\ee
where $V$ is a typical values of the electric potential produced by the central engine and  ${\cal{R} }\approx 1/ c$ is  the impedance of free space. 
In case of Crab flares, the available potential,
\be
V \sim \sqrt{L /c} \approx 1.7 \times 10^{15} \, {\rm V},
\ee 
corresponds to $\gamma \approx 3.4 \times 10^9$ - very close to the estimate (\ref{b1}). 

Similarly, the electric current associated with  flares
\be
I \approx \sqrt{L  c} \approx 5 \times 10^{22} \, {\rm cgs\, units} =  1.7 \times 10^{13} \, {\rm Ampers}
\ee
is similar to the  \Alfven current (\ref{IA})
 for the required \Lf\ (\ref{b1}):
\be
I_A =  1.7 \times 10^{23} , {\rm cgs\,  units} =  6\times 10^{13} \, {\rm Ampers}
\ee

This is important: the \Lf\ that we  derived from radiation modeling (from the peak energy and duration of flares) nearly coincides with the expected \Lf\ of particles derived from the assumption that the radiated power is similar to the intrinsic \EM\ power  of flares. In a related ``coincidence'', the current required to produce a given  luminosity nearly coincides with the corresponding \Alfven current, calculated using the \Lf\ of the emitting particles.

These coincidences, in our view, are not accidental: they imply that flares are produced by charge-separated flow. This is indeed expected in the acceleration models based on DC-type acceleration. 
This is also consistent with our PIC simulation that show effects of  Òkinetic beamingÓ - highly anisotropic distribution of the highest energy particles. {\bf SSK: I am not quiet following the argument here.}



==> CurrentFilamentation.tex <==


\subsection{Current  filamentation} 

As the mildly relativistic  post-shock flow decelerates, it comes into a global causal contact. Once causally connected, the almost purely toroidal magnetic configuration of the nebula flow is liable to current-driven instabilities \cite[e.g.][]{begelman1998,Mizuno:2011aa}.  
As pointed out by \cite{2012MNRAS.427.1497L}, in a highly magnetized expanding post-shock flow, the flow lines are in fact focussed to the axis via the magnetic hoop-stress which can act as an additional trigger for instability.  Thereby the innermost flow reaches the recollimation point first and is expected to experience violent instability and magnetic dissipation.  
\cite{2012MNRAS.427.1497L} hence argues that the $\gamma$-ray flares originate in the polar region at the base of the observed jet/plume.  
On the one hand, the simulations of \cite{2014MNRAS.438..278P} are in agreement with this dynamical picture and show development of modes with azimuthal number $m\sim few$,  that lead to the formation of current filaments at the jet base.  On the other hand, for numerical stability, \cite{2014MNRAS.438..278P} could only study moderate polar magnetizations of $\sigma\le3$ which disfavors rapid particle acceleration.  Even without this technical limitation, for non-vanishing wind power, the axis itself cannot carry a DC Poynting flux.  Because of this, we are interested in flow lines from intermediate latitudes that acquire high sigma due to flow expansion.  



To visualize the current in the simulations, we now cut the domain by spherical surfaces and investigate current-magnitude and magnetization in the $\phi\theta$-plane,   
 Fig. \ref{fig:jr}.  
In general, the current exhibits a quadrupolar morphology, it is distributed smoothly over the polar regions and returns near the equator.  When the test-surface crosses over the termination shock, we observe an increased return-current due to the shock jump of $B_\phi$.  
Although the field is predominantly toroidal in the high sigma downstream region, perturbations from the unstable jet occasionally lead to current filaments and even reversals just downstream of the termination shock.  

With increasing distance from the termination-shock, the flow becomes more and more turbulent which leads to increased filamentation and copious sign changes of the radial current.  In the underlying simulations, the magnetization in the turbulent regions has dropped already below unity which disfavors rapid particle acceleration at distances larger than a few termination shock radii.  
It is interesting to point out that although the magnetic field injected in the model decreases gradually over a large striped region of $45^\circ$, an equatorial current sheet develops none the less in the nebula.  This can be seen in the lower panel of  Fig.\ref{fig:jr} which corresponds to a surface outside of the termination shock at $r=3\times 10^{17}\rm cm$.  
%
\begin{figure}[htbp]
\begin{center}
\includegraphics[height=4.5cm]{jrsinthetar1e17.png}
\includegraphics[height=4.5cm]{sigmar1e17.png}\\
\includegraphics[height=4.5cm]{jrsinthetar3e17.png}
\includegraphics[height=4.5cm]{sigmar3e17.png}
\caption{Distribution of  the radial current, $j_r\sin\theta$ \textit{(left)} and magnetization $\sigma$ \textit{(right)}.    Dashed contours indicate the sign changes of the current and solid contours indicate levels of $\sigma=4$.  
\textit{Top:} Sphere with $r=10^{17}\rm cm$, 
one can see formation of current filaments (\eg\ regions $\theta \approx 2.5 $ and $\phi \approx -1.5,\, -0.5$). The current direction can even reverse, (the region $\theta \approx 2.7 $,  $\phi \approx -1$). 
\textit{Bottom:} Sphere with $r=3\times 10^{17}\rm cm$.  Here the current is highly filamentary and an equatorial current-sheet has developed.  The average magnetization in the current sheet and in the turbulent flow is $<1$ but magnetically dominated regions can still be obtained ($\sigma\approx6$ at $\theta\approx1.75$, $\phi\approx-1.5$).  
}
\label{fig:jr}
\end{center}
\end{figure}
%

To better understand the geometry of the current and magnetic field, we display a representative volume rendering of the polar region in Fig. \ref{fig:filamentation}. 
In the rendering, one can see the violently unstable polar beam embedded into the more regular high-$\sigma$ region comprised of toroidal field lines.  
The plume forms downstream of this structure and is also strongly perturbed.  A part of the disrupted plume approaches the termination shock as a flux-tube.  
The presence of such a configuration where two flux tubes can come together very close to the high sigma region lets us speculate that Crab flares might originate when the right geometry (e.g. parallel flux tubes) coincides with high magnetization as present in the nebula even for moderate wind magnetization.  
For higher magnetizations of the polar beam, the mechanism described by \cite{2012MNRAS.427.1497L} could directly act also without first having to rely on enhancement of $\sigma$ via flow expansion.  Extrapolating from the moderate sigma simulations where the polar beam is highly unstable and forms a filamented current, this seems feasible at the very least.  


A targeted investigation of the Crab nebula polar flow also with higher magnetization of $\sigma$ up to 10 was performed by \cite{2013MNRAS.436.1102M} through injecting a jet into the shocked nebula ambient.  The model is appropriate for the lightyear scale plume but lacks the formation of the jet via the hoop-stress in the nebula.  
To match the kinked morphology of the observations of the plume, models with moderate bulk Lorentz factors $\Gamma=2$ are favored.  
Fragmentation of the current and highly intermittent structures also develop in the large scale flow, but with time-scales of not much less than a year.  The highest variability and potential reconnection sites are localized at the termination zone of the jet at the edge of the nebula.  At this point the magnetization has dropped considerably due to internal dissipation.  
These features speak against the large scale jet as a site for the $\gamma$-ray flares.  

 
 \subsection{Summary: what large scale simulations and observations tell us}
 
Above we discussed the theoretical implications of the observations and results of the large scale relativistic MHD simulations of the pulsar wind flows. Let us summarize. 
\begin{description} 
\item  - The flare region should be located at intermediate polar angles. Its size is a substantial fraction (few to $\sim $ 10\%) of the distance from the axis. The required acceleration potential is also a  substantial fraction (few \%) of the total potential of the wind. 
\item -  The flare region  has a macroscopic size, orders of magnitude  larger than the corresponding skin depth. 
\item  - Acceleration should proceed at nearly maximal rate, with \Ef\ of the order of \Bf\ over the whole acceleration region.
\item  - Even for mildly magnetized winds (for wind magnetization $\sigma_w \geq $ few) the post-shock flow naturally forms highly magnetized regions. 
\item - Post-shock flow is unstable to large scale current-driven instabilities that lead to the formation of current/magnetic filaments.
\end {description} 


%In conclusion, large scale simulations indicate that even for mildly magnetized winds (for wind magnetization $\sigma_w \geq $ few) the post-shock flow naturally forms highly magnetized regions.  These regions are unstable to large scale current-driven instabilities that lead to the formation of current/magnetic filaments. In the following sections we discuss a number of plasma-physical models that can lead to impulsive particle acceleration in such configurations.




==> ps-flow.tex <==
ssssssssssssssssssssssssssssssssssssssssssssssssssssss
\subsection{Post-shock flow - formation of highly magnetized regions}
\label{formationmagnetized}

The powerful Crab flares require that energy from a macroscopic scale is made available to the acceleration process.  As we will discuss in the following, current-driven MHD instabilities like the coalescence of parallel currents and the "X-point collapse" can be a viable way to achieve this.  One of the key  questions is then how a violently unstable and highly magnetized configuration is setup in the first place.  
To locate potential sites for the flaring region, we need to identify regions of high sigma and analyze the flow structure in these candidate flaring regions.  Here we use the result of simulations by \cite{2014MNRAS.438..278P}.
Although the scales required for the ``daily'' flare duration are not resolved by the simulation (its resolution is $>3$ light-days), it is instructive to correlate the high-sigma region (that forms as a consequence of flow-expansion) with the current distribution in the simulations.  

As \cite{2016MNRAS.456..286L} discuss, the modeling of the inner knot of the Crab Nebula requires that the equatorial flow is weakly magnetized. Intermediate latitudes can still be highly magnetized. 
In fact,  highly magnetized regions  in the bulk of the nebula  can be achieved via flow expansion at  intermediate latitude regions {\it starting with only mildly magnetized wind}. In  Fig. \ref{fig:overview} we show the magnetization in the $xy$-plane from simulations of \citep{2014MNRAS.438..278P}.  One can clearly see that the magnetization rises well above the maximal injected value of $\sigma=1$.  The highest value of $\sigma\approx8$ in the snapshot is achieved at the point where radial expansion reverses and forms the plume-like polar flow.  
%It should be pointed out that the high-sigma region can be separated clearly from the inner knot  \cite{2016MNRAS.456..286L} which requires a magnetization of $\sigma\ll 1$ for the successful modeling of the termination shock emission as illustrated in Fig. \ref{fig:overview}, (right panel).  
%
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.4\textwidth]{sigma-surfaces0501.png}
\includegraphics[width=0.4\textwidth]{sigma.pdf}
\caption{{\it Left panel}. Magnetization in the $yz$ plane, also indicating the location of the spherical cut as a white circle.  The radius is  $r =  10^{17}\rm cm$.  {\it Right panel}. Zoom-in on the central part. The dashed line
is the line of view and the blue curves show the regions of enhanced
observed emissivity \citep[the inner knot][]{2016MNRAS.456..286L}. The dot-dashed line separates the high and low
magnetization regions of the wind.  The arrowed lines are the instantaneous stream lines.  Red line if the position of the shock. There is a clearly visible region of high magnetization at intermediate latitudes.}
\label{fig:overview}
\end{center}
\end{figure}
%

To understand the formation of highly magnetized regions starting with only mildly magnetized conditions at the reverse shock, Fig. \ref{fig:overview},  let us consider the post oblique shock evolution of the wind.
 Let the wind magnetization be $\sigma_w \gtrsim  1$, Eq.  (\ref{sigmaw}), and wind Lorentz factor $\gamma_w\gg 1$.  Let us consider evolution of plasma magnetization in the post-shock flow. Magnetization first changes at the shock. As a guide we can use solutions for the normal shocks \citep{kc84} -  in oblique relativistic shocks the compression ratio differs considerably from that of the normal shock only for very small angles of attack \citep[see, \eg Fig.  A2 of ][]{2016MNRAS.456..286L}. In the $\sigma_w \gg 1$ case the post-shock magnetization parameter, defined in terms of the ratio of the magnetic energy to plasma enthalpy, is 
$\sigma = 2 \sigma _w$, while  typical thermal Lorentz factor is $\gamma_T \approx \gamma_w /( 8 \sqrt{\sigma_w})$ \citep{kc84,2007A&A...473..683P}.  
 Note, that magnetization  increases  at the shock -  $\sigma$ is the measure of the ratio of the magnetic energy density to plasma energy density in the flow frame;  in a highly magnetized strong shock the rest-frame \Bf\ increases due to flow deceleration (observer-frame \Bf\ remains nearly the same). This increase if rest-frame \Bf\ over-compensates the dissipated part 
of the magnetic energy.
 At the same time the post-shock \Lf\ is $\gamma_2 \sim \sqrt{\sigma_w}/\sin \delta_1$,
where $\delta_1 \sim 0.1-0.5$ is the angle of attack. This value can reach $\sim$ tens for $\sigma_w \geq 100$; as a conservative lower limit let us use $\gamma_2 \geq 10$. 
 


As a highly relativistic, $\gamma_2\gg 1$ flow propagates into the nebula, it is decelerated by the nebular material. As long as it remains relativistic, the flow remains nearly radial  \citep[also, for $\sigma \gg 1$ the deflection angle at the shock is small][]{2012MNRAS.422.3118L,2016MNRAS.456..286L}.  As a result of deceleration the  magnetic field is further amplified within the nebula   \citep[the Cranfill effect][]{cran71}, leading to formation of high-$\sigma$ regions even for mild pre-shock magnetization. 

The increased magnetization regions within the nebula are clearly seen in numerical simulations. For example, in Fig. \ref{fig:overview} we show plasma magnetization in simulations of \citet{2014MNRAS.438..278P}.  A high $\sigma$ region  originates from smaller $\sigma$ parts of the wind (in  the simulations that part of the wind  has $\sigma_w=3$), then $\sigma$ gets amplified at the shock, and later on  it gets even more amplified in the bulk. At the same time the bulk Lorentz factor decreases, while the flow trajectory becomes substantially non-radial. Thus, {\it creation of highly magnetized regions, even starting from mildly magnetized flows, is a natural consequence of flow evolution within the nebula.}

Guided by the results of the numerical simulations \citep[which used mild magnetization and wind Lorentz factors][]{2013MNRAS.431L..48P}, we can estimate the general behavior of the post-shock flow. Simulations show that, approximately,  in doubling the radius, the flow decelerates from highly relativistic  post-shock value, $\gamma_2 \gg 1$, to  a non-relativistic  one $v/c\sim  0.1$, while the enthalpy drops by a factor of a few. This must  results in a huge increase of the rest-frame \Bf\ and plasma magnetization, as we discuss next. 
From the induction equation $B \Gamma r v\approx $ constant for quasi-stationary radial flow, the  \Bf\  $B_f$ in the flare region can be estimated as 
\be
B_f \approx  \left( { r_s \over r_f} \right)\left( { c \over v_f} \right) \Gamma_2 B_2
\ee
where $r_s$ is a shock radius along a given flow line, $B_2$ is a value of the \Bf\ at the shock,  $ \Gamma_2$ is the immediate post-shock Lorentz factor; $B_f, \, r_f, \, v_f$ are evaluated in the flare region.  Since  $r_f/r_s \sim 2$, while  $\Gamma_2 \approx \sqrt{\sigma_w}/\delta_1  \gg 1$ and $c/v_f \sim  $ few, we find that the rest-frame \Bf\ in the flare region may {\it exceeds} the values at the shock. At the same time,   density (from $\rho \Gamma r^2 v \approx $ constant)  is
\be
\rho_f \approx  \left( { r_s \over r_f} \right)^2 \left( { c \over v_f} \right)  \Gamma_2  \rho_s.
\ee
For relativistic fluid with adiabatic index of $4/3$ the magnetization in the flare region is then related to the magnetization at the shock $\sigma_2$ and in the wind $\sigma_w$ as
\be
\sigma_f=  \left( { r_f \over r_s} \right)^{2/3} \left( { c \over v_f} \right) ^{2/3} \Gamma_2^{2/3} \sigma_2 
%= 8 \left( { r_s \over r_f} \right)^{14/3} \left( { c \over v_f} \right) ^{2/3} \Gamma_2^{2/3} \sigma_w
\label{sigmaf}
\ee
(here $\sigma$ is defined as the ratio of  two times the magnetic energy to enthalpy, assuming highly relativistic EoS).
%where the last relation assumes $\sigma_w \gg 1$.
All factors in Eq. (\ref{sigmaf}) in front of the shock magnetization parameter $\sigma_2$ are  larger than unity, thus $\sigma_f \gg \sigma_2 $.  Thus, even for $\sigma_w \sim $ few, there is strong amplification of $\sigma$ right at the shock (by as much as a factor of 2, $\sigma_2 \sim 2 \sigma_w$), and then another amplification in the bulk, $\sigma_f \gg \sigma_2 $.


Based on the above discussion, we expect that in the post-shock flow the magnetization may increase by a  large value. Though the above considerations are approximate, and neglect a number of important details (most importantly, the development of non-radial and non-axisymmetric velocity field), the expected effect  -  a large growth of the magnetization, is huge. Thus, we conclude that   highly magnetized structures are naturally formed in the post-shock flow. 



\subsection{Current  filamentation} 

As the mildly relativistic  post-shock flow decelerates, it comes into a global causal contact. Once causally connected, the almost purely toroidal magnetic configuration of the nebula flow is liable to current-driven instabilities \cite[e.g.][]{begelman1998,Mizuno:2011aa}.  
As pointed out by \cite{2012MNRAS.427.1497L}, in a highly magnetized expanding post-shock flow, the flow lines are in fact focussed to the axis via the magnetic hoop-stress which can act as an additional trigger for instability.  Thereby the innermost flow reaches the recollimation point first and is expected to experience violent instability and magnetic dissipation.  
\cite{2012MNRAS.427.1497L} hence argues that the $\gamma$-ray flares originate in the polar region at the base of the observed jet/plume.  
On the one hand, the simulations of \cite{2014MNRAS.438..278P} are in agreement with this dynamical picture and show development of modes with azimuthal number $m\sim few$,  that lead to the formation of current filaments at the jet base.  On the other hand, for numerical stability, \cite{2014MNRAS.438..278P} could only study moderate polar magnetizations of $\sigma\le3$ which disfavours rapid particle acceleration.  Even without this technical limitation, for non-vanishing wind power, the axis itself cannot carry a DC Poynting flux.  Because of this, we are interested in flow lines from intermediate latitudes that acquire high sigma due to flow expansion.  

To visualize the current in the simulations, we now cut the domain by spherical surfaces and investigate current-magnitude and magnetization in the $\phi\theta$-plane.  
The white circles in Fig. \ref{fig:overview} indicates the location of the innermost spherical test-surface shown in the top panel of Fig. \ref{fig:jr}.  
In general, the current exhibits a quadrupolar morphology, it is distributed smoothly over the polar regions and returns near the equator.  When the test-surface crosses over the termination shock, we observe an increased return-current due to the shock jump of $B_\phi$.  
Although the field is predominantly toroidal in the high sigma downstream region, perturbations from the unstable jet occasionally lead to current filaments and even reversals just downstream of the termination shock.  

With increasing distance from the termination-shock, the flow becomes more and more turbulent which leads to increased filamentation and copious sign changes of the radial current.  In the underlying simulations, the magnetization in the turbulent regions has dropped already below unity which disfavours rapid particle acceleration at distances larger than a few termination shock radii.  
It is interesting to point out that although the magnetic field injected in the model decreases gradually over a large striped region of $45^\circ$, an equatorial current sheet develops none the less in the nebula.  This can be seen in the lower panel of  Fig.\ref{fig:jr} which corresponds to a surface outside of the termination shock at $r=3\times 10^{17}\rm cm$.  
%
\begin{figure}[htbp]
\begin{center}
\includegraphics[height=4.5cm]{jrsinthetar1e17.png}
\includegraphics[height=4.5cm]{sigmar1e17.png}\\
\includegraphics[height=4.5cm]{jrsinthetar3e17.png}
\includegraphics[height=4.5cm]{sigmar3e17.png}
\caption{Distribution of  the radial current, $j_r\sin\theta$ \textit{(left)} and magnetization $\sigma$ \textit{(right)}.    Dashed contours indicate the sign changes of the current and solid contours indicate levels of $\sigma=4$.  
\textit{Top:} Sphere with $r=10^{17}\rm cm$, 
one can see formation of current filaments (\eg\ regions $\theta \approx 2.5 $ and $\phi \approx -1.5,\, -0.5$). The current direction can even reverse, (the region $\theta \approx 2.7 $,  $\phi \approx -1$). 
\textit{Bottom:} Sphere with $r=3\times 10^{17}\rm cm$.  Here the current is highly filamentary and an equatorial current-sheet has developed.  The average magnetization in the current sheet and in the turbulent flow is $<1$ but magnetically dominated regions can still be obtained ($\sigma\approx6$ at $\theta\approx1.75$, $\phi\approx-1.5$).  
}
\label{fig:jr}
\end{center}
\end{figure}
%

To better understand the geometry of the current and magnetic field, we display a representative volume rendering of the polar region in Fig. \ref{fig:filamentation}. 
In the rendering, one can see the violently unstable polar beam embedded into the more regular high-$\sigma$ region comprised of toroidal field lines.  
The plume forms downstream of this structure and is also strongly perturbed.  A part of the disrupted plume approaches the termination shock as a flux-tube.  
The presence of such a configuration where two flux tubes can come together very close to the high sigma region lets us speculate that Crab flares might originate when the right geometry (e.g. parallel flux tubes) coincides with high magnetization as present in the nebula even for moderate wind magnetization.  
For higher magnetizations of the polar beam, the mechanism described by \cite{2012MNRAS.427.1497L} could directly act also without first having to rely on enhancement of $\sigma$ via flow expansion.  Extrapolating from the moderate sigma simulations where the polar beam is highly unstable and forms a filamented current, this seems feasible at the very least.  

%
\begin{figure}[htbp]
\begin{center}
\includegraphics[height=10cm]{Currentfilaments.png}
\caption{3D volume rendering showing current filamentation of the polar beam just downstream of the termination shock.  The shock surface is indicated as the orange plane and we draw field-lines shaded from white $(\sigma=0)$ to black ($\sigma=5$).  
One clearly sees two current filaments producing structures similar to magnetic flux tubes.  As discussed in \cite{2014MNRAS.438..278P}, streamlines from intermediate latitudes reach the axis behind this inner violently unstable region and form a plume-like outflow of moderate velocity $v\approx0.7c$.  
}
\label{fig:filamentation}
\end{center}
\end{figure}
%

A targeted investigation of the Crab nebula polar flow also with higher magnetization of $\sigma$ up to 10 was performed by \cite{2013MNRAS.436.1102M} through injecting a jet into the shocked nebula ambient.  The model is appropriate for the lightyear scale plume but lacks the formation of the jet via the hoop-stress in the nebula.  
To match the kinked morphology of the observations of the plume, models with moderate bulk Lorentz factors $\Gamma=2$ are favored.  
Fragmentation of the current and highly intermittent structures also develop in the large scale flow, but with time-scales of not much less than a year.  The highest variability and potential reconnection sites are localized at the termination zone of the jet at the edge of the nebula.  At this point the magnetization has dropped considerably due to internal dissipation.  
These features speak against the large scale jet as a site for the $\gamma$-ray flares.  

 
 \subsection{Summary: what large scale simulations and observations tell us}
 
Above we discussed the theoretical implications of the observations and results of the large scale relativistic MHD simulations of the pulsar wind flows. Let us summarize. 
\begin{description} 
\item  - The flare region should be located at intermediate polar angles. Its size is a substantial fraction (few to $\sim $ 10\%) of the distance from the axis. The required acceleration potential is also a  substantial fraction (few \%) of the total potential of the wind. 
\item -  The flare region  has a macroscopic size, orders of magnitude  larger than the corresponding skin depth. 
\item  - Acceleration should proceed at nearly maximal rate, with \Ef\ of the order of \Bf\ over the whole acceleration region.
\item  - Even for mildly magnetized winds (for wind magnetization $\sigma_w \geq $ few) the post-shock flow naturally forms highly magnetized regions. 
\item - Post-shock flow is unstable to large scale current-driven instabilities that lead to the formation of current/magnetic filaments.
\end {description} 




 
